Acoustic span embeddings for multilingual query-by-example search

Query-by-example (QbE) speech search is the task of matching spoken queries to utterances within a search collection. In low- or zero-resource settings, QbE search is often addressed with approaches based on dynamic time warping (DTW). Recent work has found that methods based on acoustic word embeddings (AWEs) can improve both performance and search speed. However, prior work on AWE-based QbE has primarily focused on English data and with single-word queries. In this work, we generalize AWE training to spans of words, producing acoustic span embeddings (ASE), and explore the application of ASE to QbE with arbitrary-length queries in multiple unseen languages. We consider the commonly used setting where we have access to labeled data in other languages (in our case, several low-resource languages) distinct from the unseen test languages. We evaluate our approach on the QUESST 2015 QbE tasks, finding that multilingual ASE-based search is much faster than DTW-based search and outperforms the best previously published results on this task.

==> approach_old.tex <==
\section{MULTILINGUAL EMBEDDING-BASED QbE}
\label{sec:approach}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/architecture.png}
    \caption{(a) Contextualized acoustic word embedding (AWE) model $f_w$ and acoustically grounded word embedding (AGWE) model $g_w$. (b) Acoustic span embedding (ASE) model $f_s$ and acoustically grounded span embedding (AGWE) model $g_s$. \klcomment{Need to clarify what the "pre-trained AWE" and "pre-trained AGWE" layers are.  It could be nice to have a single figure that combines the AWE and ASE/APE, though it might be hard to do.}}
    \label{fig:ase}
    \vspace{-0.5cm}
\end{figure}

%Similar to~\cite{settle2017query},
Our embedding-based QbE system consists of an embedding method and a search component.
Similar to~\cite{hu2020multilingual}, we jointly train acoustic word embeddings (AWE) and acoustically grounded word embeddings (AGWE) for use in QbE search. To limit mismatch between AWE training and QbE evaluation, we modify AWE+AGWE training to include contextual information, and we also extend training to single and multi-word spans through joint learning of acoustic span embedding (ASE) and acoustically grounded span embedding (AGSE) models.

\subsection{Multilingual acoustic word embedding with context}
\label{ssec:awe}
Our multilingual AWE method is based on~\cite{hu2020multilingual} where we jointly learn two embedding models: an acoustic-view ($f_w$) and a written-view ($g_w$). The acoustic-view model maps an arbitrary-length spoken word segment to a fixed-dimensional vector, while the written-view model $g_w$ maps the word's corresponding phone sequence to another fixed-dimensional vector. Word-level alignments $\mathcal{A} = \{(s_1, e_1, w_1), ..., (s_L, e_L, w_L)\}$ where each tuple $(s_i, e_i, w_i)$ indicates start frame, end frame, and word label for segment $i$ are used. In prior work~\cite{he+etal_iclr2017,hu2020multilingual}, these alignments $\mathcal{A}$ are used to extract isolated word segments before they are passed through $f_w$. In this work, we input full utterances ${\bf X} \in \mathbb{R}^{T \times D}$ to the acoustic-view model $f_w$ to incorporate contextual information. A separate embedding is then produced for each segment in the corresponding alignment $\mathcal{A}$. These embeddings are derived from
%In prior work~\cite{he+etal_iclr2017,hu2020multilingual}, word-level alignments are used to extract isolated word segments before forwarding them through $f$. In this work, we use contextual AWEs (see Figure~\ref{fig:ase}). Full utterances are input the acoustic-view model $f_w$ and the embedding of each word segment $i$ is derived from %hidden state outputs and $L$ word-level alignments $\{(s_1, e_1, w_1), ..., (s_L, e_L, w_L)\}$ where $(s_i, e_i, w_i)$ indicates the start frame, end frame, and word label for segment $i$. For consistency with Equation~\ref{eq:mv}, word segment $i$'s embedding $f({\bf X}_i)$ is computed using
either the {\bf average} of the aligned output hidden states $s_i$ to $e_i$
\begin{flalign*}
    f_w^{avg}({\bf X}_i) &= \frac{1}{e_i - s_i + 1} \sum_{j={s_i}}^{e_i} f_w({\bf X})_j \text{ where } f_w({\bf X}) \in \mathbb{R}^{T \times d}
\end{flalign*}
or {\bf concatenation} of the forward hidden state $e_i$ and backward hidden state $s_i$
\begin{flalign*}
    f_w^{cat}({\bf X}_i) &= \left[ f_w({\bf X})_{e_i}^{\rightarrow}; f_w({\bf X})_{s_i}^{\leftarrow} \right] \text{ where } f_w({\bf X}) \in \mathbb{R}^{T \times d}
\end{flalign*}
%The acoustic-view model $f_w$ maps an arbitrary-length spoken word segment ${\bf X}_i \in \mathbb{R}^{T \times D}$ to a fixed-dimensional vector $f_w({\bf X}_i) \in \mathbb{R}^d$, while the written-view model $g_w$ maps the word's corresponding phone sequence ${\bf p}_i$ to another vector $g_w({\bf p}_i) \in \mathbb{R}^d$.
\ssedit{Contextualized AWEs improve performance~\cite{yuan2018learning} \klcomment{changed this citation to one at a higher-profile venue; if there is something different and important in~\cite{yuan2019recurrent}, though, we can change it back} over isolated word segments, allow for straightforward extension to ASE training on single and multi-word spans (see Section~\ref{ssec:ape}), and give speed benefits when embedding queries as well as utterances from the search collection.} The written-view $g_w$ is used identically to~\cite{hu2020multilingual}. We use the same BiGRU~\cite{cho2014learning} architecture as described in~\cite{hu2020multilingual} for $f_w$ and $g_w$. The training objective used in~\cite{hu2020multilingual} is given minor updates to improve word discrimination performance. \klcomment{can we say more about the effect of contextualized vs. isolated-word embeddings, and of the updated objective?  can we report results showing the effects of these?}\yhcomment{First, Contextualized AWE supports the further fine-tuning with phrases. The second concern is speed. Contextualized-AWE only has to embed each utterance once. We should write about it here clearly.It also has some benefits in performance, although we have not measured it. } Training consists of minimizing the following objective where $f$ and $g$ are given by $f_w^{avg}$ (or $f_w^{cat}$) and $g_w$, respectively:
\begin{flalign}
\sum_{n=1}^{N}\sum_{i=1}^{L_n}\sum_{k=0}^{2}&\left[
        m + d(f({\bf X}_i^{(n)}), g(v_i^{(n)})) - d_k^{\star}({\bf X}_i^{(n)}, v_i^{(n)})
    \right]_{+}\notag\\
    %+&\left[
    %    m + d(g(v_i), f({\bf X}_i)) - d_1^{\star}({\bf X}_i, v_i)
    %\right]_{+}\notag\\
    %+&\left[
    %    m + d(g(v_i), f({\bf X}_i)) - d_2^{\star}({\bf X}_i, v_i)
    %\right]_{+}
\label{eq:mv}
\end{flalign}
To improve performance and efficiency, we conduct semi-hard negative sampling~\cite{schroff2015facenet} given each training pair $({\bf X}, v)$:
\begin{flalign*}
    d_0^{\star}({\bf X}, v) &= \displaystyle \min_{v' \in \mathcal{V}_0'({\bf X}, v)} d(f({\bf X}), g(v'))\\
    d_1^{\star}({\bf X}, v) &= \displaystyle \min_{v' \in \mathcal{V}_1'({\bf X}, v)} d(g(v), g(v'))\\
    d_2^{\star}({\bf X}, v) &= \displaystyle \min_{{\bf X}' \in \mathcal{X}_2'({\bf X}, v)} d(g(v), f({\bf X}'))
\end{flalign*}
where
\begin{flalign*}
    \mathcal{V}_0'({\bf X}, v) &:= \{
        v' \vert d(f({\bf X}), g(v')) > d(f({\bf X}), g(v)), v' \in \mathcal{V} / v
    \}\\
        \mathcal{V}_1'({\bf X}, v) &:= \{
        v' \vert d(g(v), g(v')) > d(g(v), f({\bf X})), v' \in \mathcal{V} / v
    \}\\
    \mathcal{X}_2'({\bf X}, v) &:= \{
        {\bf X}' \vert d(g(v), f({\bf X}')) > d(g(v), f({\bf X})), v' \in \mathcal{V} / v 
    \}
\end{flalign*}
${\bf X_i}$ is a spoken word segment, $v_i$ is its word label,
$m$ is a margin hyperparameter, $d$ denotes cosine distance $d(a,b) = 1-\frac{a\cdot b}{\Vert a \Vert\Vert b \Vert}$, $N$ is the number of training pairs, and $\mathcal{V}$ is the training vocabulary. This objective encourages embedding spoken word segments corresponding to the same word label close together and close to their learned label embeddings, while ensuring that segments corresponding to different word labels are mapped farther apart (and nearer to their respective label embeddings).
%and using the concatenated first and last hidden states as our embedding vector,  The only difference is the input to $f_w$. In prior work~\cite{he+etal_iclr2017,hu2020multilingual}, the input to $f_w$ is a single isolated spoken word segment. In this work, to accelerate the embedding approach in QbE tasks, $f_w$ takes %an arbitrary-length
%the full utterance as input and generates a separate acoustic embedding for each word.
%in the utterance at the same time.
%For an utterance $\bf{X} \in \mathbb{R}^{T \times D}$, where $T$ is the number of frames and $D$ is the acoustic feature dimension, we consider two ways of computing the embedding vector 
%In detail, let the utterance be $\bf{X} \in \mathbb{R}^{T \times D}$, where $T$ is the number of frames and $D$ is the dimension of the acoustic feature. Let $\bf x_i$ be the speech segment of a word in the utterance. $\bf x_i$ starts at $t_{i}^{start}$ and ends at  $t_{i}^{end}$, in which $0 \le t_{i}^{start} < t_{i}^{end} \le T$. We consider two ways to compute the embedding vector $f_w(\bf x_i)$.
%\begin{itemize}
%    \item \textbf{Mean}: we concatenates the mean of the outputs in time steps $[t_{i}^{start}, t_{i}^{end}]$ of the top layer in both directions of the BiGRU network as the fixed-dimensional embedding.
%    \item \textbf{Concat}: We concatenate the output at time step $t_{i}^{end}$ in the forward direction and the output at time step $t_{i}^{start}$  in the backward direction in the top layer of the BiGRU network as the fixed-dimensional embedding.
%\end{itemize}
%The written-view model $g_w$, training objective, and all other details are the same as~\cite{hu2020multilingual}.

\subsection{Acoustic spans embedding}
\label{ssec:ape}
\klcomment{This section is hard to follow.  To help organize this section, I suggest writing down a formal algorithm that takes in training data and outputs the learned APE/AGPE models.  Then we could include the algorithm itself, or distill it into a text description.}
To overcome the mismatch between AWE training and QbE search evaluation, we extend AWE+AGWE~\cite{hu2020multilingual} training to allow single and multi-word spans. Joint learning of span-level acoustic-view model ($f_s$) and written-view model ($g_s$).
%While the multilingual AWE model is trained to embed speech segments corresponding to single words, QbE search we require embedding spoken queries which span multiple words into a single fixed-dimensional vector. To address this mismatch, we extend our AWE method~\cite{he+etal_iclr2017,hu2020multilingual} to acoustic phrase embedding (APE), which involves jointly training a phrase-level acoustic-view model ($f_p$) and a phrase-level written-view model ($g_p$).

%Given a variable-length spoken segment ${\bf X} \in \mathbb{R}^{T \times D}$, $f_p$ maps the ${\bf X}$ to a vector $f_p({\bf X}) \in \mathbb{R}^d$, but in this case, the speech segment may contain multiple words. $g_p$ is trained to map a word sequence into the same hidden space as $f_p$. The goal is to learn $f_p$ and $g_p$ jointly such that instances of both speech segments and their corresponding written word sequences are mapped close together, while instances with different transcription are kept apart.

During word-level training, alignments $\{(s_1, e_1, w_1), ..., (s_L, e_L, w_L)\}$ are used such that acoustic word embeddings can be extracted from $f_w({\bf X}_{s_i:e_i})$. The same word-level alignments are used when training both AWE models and ASE models, the only difference is that during ASE training 

As shown in Figure~\ref{fig:ase}, our ASE model uses the multilingual AWE model as a building block. For a pair of word-level models $f_w$ and $g_w$ pre-trained following Section~\ref{ssec:awe}, we jointly learn $f_p$ and $g_p$ on top of these pre-trained word-level models. The acoustic-view phrase embedding model $f_p$ uses $f_w$ supplemented with additional layers. $f_p$ generates acoustic embeddings for segments similarly to $f_w$ as discussed in~\ref{ssec:awe} (i.e. {\bf mean} or {\bf concat}), except that alignments are randomized such that segment end times are ignored with probability $p$. If $p=0$, then all segment embeddings can be considered word-level. If $p \in (0, 1)$, then some segment embeddings will pertain to multi-word phrases, and in Equation~\ref{fig:mv} training pairs $({\bf X}_i, v_i)$ refer to sampled phrase segments rather than individual words. In this setting, $f$ and $g$ are given by $f_p$ and $g_p$, respectively, in Equation~\ref{eq:mv}. %The only difference is that now an alignment may multiple words may appear in the speech segment.
The written-view model $g_p$ takes the sampled single-word or multi-word sequences described above as input. For example, given a word sequence $w_1, w_2, ..., w_L$, $g_p$ (a single layer BiGRU network) accepts input written-view word embeddings $g_w(w_1), g_w(w_2),..., g_w(w_L)$ as input. The phrase-level written-view embedding consists of a concatenation of the last forward hidden state and the first backward hidden state of the BiGRU network $g_p$ (similar to $g_w$).

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/QbE.png}
  \caption{QbE search with acoustic embeddings.  \klcomment{we may want to switch this fig with fig. 2, since fig. 2 represents the innovation in this paper, whereas this one is similar to figures in multiple other papers}
  }
\label{fig:qbe_system}
\end{figure}



\subsection{Embedding-based QbE with sliding window}
\label{ssec:embqbe}
Figure~\ref{fig:qbe_system} shows our multilingual embedding-based QbE system. Given a pre-trained acoustic embedding model, we first build an index of the utterances by embedding all possible segments. Similar to~\cite{yuan2018learning}, we use a simple sliding window algorithm to choose the possible segments, and we choose several window sizes according to the range of query length. %We apply the windows on the time axis of the utterances.
The speech segment in the analysis window is then mapped to an embedding vector by our embedding model. %Notice that this process is really fast since our AWE and APE models takes the whole utterance as input and can generate the acoustic embeddings of all possible segments in the utterance at the same time.
Given an audio query, we first embed the query with the same pre-trained embedding model. Then we compute a detection score between the query and each search utterance via cosine similarity:
\begin{equation}
    score(q,S) = \underset{s \in S_T}{max}{\frac{f(s) \cdot f(q)}{||f(s)||_2||f(q)||_2}}
\label{eq:score}
\end{equation}
where $q$ is the query, $S$ is the search utterance, $S_T$ is the set of all possible segments in $S$. $f$ is the acoustic embedding function. The higher the score, the more probability that the query matches the search utterance.
